Symbol Detection for Frame-Based Faster-than-Nyquist Signaling via Sum-of-Absolute-Values Optimization

In this letter, we propose a new symbol detection method for faster-than-Nyquist signaling (FTNS) systems. Based on frame theory, we formulate a symbol detection problem as a under-determined linear equation on a finite set. The problem is reformulated as a sum-of-absolute-values (SOAV) optimization that can be efficiently solved by the fast iterative shrinkage thresholding algorithm (FISTA). The proximity operator for the convex optimization is derived analytically. Simulation results are given to show that the proposed method can successfully detect symbols in faster-than-Nyquist signaling systems and has lower complexity in terms of computation time.

==> Fig/prox.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(28.0000,20.6500)(6.0000,-22.0000)%
% LINE 2 0 3 0 Black White  
% 2 2000 200 2000 2200
% 
\special{pn 8}%
\special{pa 2000 200}%
\special{pa 2000 2200}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 1600 1600 2400 800
% 
\special{pn 20}%
\special{pa 1600 1600}%
\special{pa 2400 800}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 2400 800 2800 800
% 
\special{pn 20}%
\special{pa 2400 800}%
\special{pa 2800 800}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 2800 800 3400 200
% 
\special{pn 20}%
\special{pa 2800 800}%
\special{pa 3400 200}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 1600 1600 1200 1600
% 
\special{pn 20}%
\special{pa 1600 1600}%
\special{pa 1200 1600}%
\special{fp}%
% LINE 0 0 3 0 Black White  
% 2 1200 1600 600 2200
% 
\special{pn 20}%
\special{pa 1200 1600}%
\special{pa 600 2200}%
\special{fp}%
% LINE 2 0 3 0 Black White  
% 2 600 1200 3400 1200
% 
\special{pn 8}%
\special{pa 600 1200}%
\special{pa 3400 1200}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 1200 1000 1200 1100 5 0 0 0
% \large{$-2$}
\put(12.0000,-11.0000){\makebox(0,0){\large{$-2$}}}%
% STR 2 0 3 0 Black White  
% 4 1600 1000 1600 1100 5 0 0 0
% \large{$-1$}
\put(16.0000,-11.0000){\makebox(0,0){\large{$-1$}}}%
% STR 2 0 3 0 Black White  
% 4 2100 1200 2100 1300 5 0 0 0
% \large{$O$}
\put(21.0000,-13.0000){\makebox(0,0){\large{$O$}}}%
% STR 2 0 3 0 Black White  
% 4 2400 1200 2400 1300 5 0 0 0
% \large{$1$}
\put(24.0000,-13.0000){\makebox(0,0){\large{$1$}}}%
% STR 2 0 3 0 Black White  
% 4 2800 1200 2800 1300 5 0 0 0
% \large{$2$}
\put(28.0000,-13.0000){\makebox(0,0){\large{$2$}}}%
% STR 2 0 3 0 Black White  
% 4 1900 700 1900 800 5 0 0 0
% \large{$1$}
\put(19.0000,-8.0000){\makebox(0,0){\large{$1$}}}%
% LINE 2 2 3 0 Black White  
% 2 2400 1200 2400 800
% 
\special{pn 8}%
\special{pa 2400 1200}%
\special{pa 2400 800}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 2800 800 2800 1200
% 
\special{pn 8}%
\special{pa 2800 800}%
\special{pa 2800 1200}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 2400 800 2000 800
% 
\special{pn 8}%
\special{pa 2400 800}%
\special{pa 2000 800}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 1600 1200 1600 1600
% 
\special{pn 8}%
\special{pa 1600 1200}%
\special{pa 1600 1600}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 1200 1600 1200 1200
% 
\special{pn 8}%
\special{pa 1200 1600}%
\special{pa 1200 1200}%
\special{dt 0.045}%
% LINE 2 2 3 0 Black White  
% 2 1600 1600 2000 1600
% 
\special{pn 8}%
\special{pa 1600 1600}%
\special{pa 2000 1600}%
\special{dt 0.045}%
% STR 2 0 3 0 Black White  
% 4 2100 1500 2100 1600 5 0 0 0
% \large{$-1$}
\put(21.0000,-16.0000){\makebox(0,0){\large{$-1$}}}%
% STR 2 0 3 0 Black White  
% 4 3400 1000 3400 1100 5 0 0 0
% \large{$\alpha$}
\put(34.0000,-11.0000){\makebox(0,0){\large{$\alpha$}}}%
% STR 2 0 3 0 Black White  
% 4 2200 100 2200 200 5 0 0 0
% \large{$\xi(\alpha)$}
\put(22.0000,-2.0000){\makebox(0,0){\large{$\xi(\alpha)$}}}%
\end{picture}}%

